Query K-means Clustering and the Double Dixie Cup Problem

We consider the problem of approximate $K$-means clustering with outliers and side information provided by same-cluster queries and possibly noisy answers. Our solution shows that, under some mild assumptions on the smallest cluster size, one can obtain an $(1+\epsilon)$-approximation for the optimal potential with probability at least $1-\delta$, where $\epsilon>0$ and $\delta\in(0,1)$, using an expected number of $O(\frac{K^3}{\epsilon \delta})$ noiseless same-cluster queries and comparison-based clustering of complexity $O(ndK + \frac{K^3}{\epsilon \delta})$, here, $n$ denotes the number of points and $d$ the dimension of space. Compared to a handful of other known approaches that perform importance sampling to account for small cluster sizes, the proposed query technique reduces the number of queries by a factor of roughly $O(\frac{K^6}{\epsilon^3})$, at the cost of possibly missing very small clusters. We extend this settings to the case where some queries to the oracle produce erroneous information, and where certain points, termed outliers, do not belong to any clusters. Our proof techniques differ from previous methods used for $K$-means clustering analysis, as they rely on estimating the sizes of the clusters and the number of points needed for accurate centroid estimation and subsequent nontrivial generalizations of the double Dixie cup problem. We illustrate the performance of the proposed algorithm both on synthetic and real datasets, including MNIST and CIFAR $10$.

==> arya_alg.tex <==
The algorithm presented in \cite{mazumdar2017clustering} is shown in Algorithm \ref{alg:AryaNoisy}. Parameters and functions that used in the algorithm are defined as: $N=\frac{64k^2\log(n)}{(1-2p)^4},c=\frac{16}{(1-2p)^2},T(a)=pa+\frac{6\sqrt{N\log(n)}}{(1-2p)},\theta(a)=2p(1-p)a+2\sqrt{N\log(n)}$, where $k$ is the number of clusters, $n$ is the number of data points and $p$ is the error probability. For a weighted graph $G(V,E)$, let $N^{+}(u)$ denote all the neighbors of $u$ in $V'$ that are connected with $u$ by $+1$ weight edge.
\begin{algorithm2e}
\caption{Clustering with noisy oracle $\mathcal{O}_n$}
\label{alg:AryaNoisy}
\SetAlgoLined
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInput{Phaseone}{Phase 1}
\SetKwInput{Phasetwo}{Phase 2}
\SetKwInput{Phasethree}{Phase 3}
\SetKwInput{Mainalgo}{Main Algorithm}

  \Input{A set of $n$ points $V$, number of clusters $k$, noisy oracle $\mathcal{O}_n$, error probability $p$. 
  }
  \Output{all clusters in \emph{active}, which have sizes at least $\Omega(\frac{k\log(n)}{(1-2p)^4})$.
  }
  \Mainalgo{\;
      \textbf{Initialization}: Initially we have an empty graph $G'=(V',E')$, and all vertices in $V$ are unassigned to any cluster. The cluster set \emph{active} is empty.\;
      \Phaseone{Selecting a small subgraph.\;
      Add new vertices uniformly at random from the unassigned vertices in $V \backslash V'$ to $V'$ making sure that the size of $V'$ is $N$. If there are not enough vertices left in $V \backslash V'$ to $V'$, select all of them.\;
      Update the weights for $G(V',E')$ by querying the oracle. For each pair $(u,v)$, $w(u,v)=+1$ if the answer is yes and $-1$ otherwise.\;
      }
      \Phasetwo{Finding active clusters\;
      \For{each pair $(u,v)$ in $V'$ and $u\neq v$}{
          \uIf{$|N^+(u)|\geq T(|V'|)$ and $|N^+(v)|\geq T(|V'|)$ and $|N^+(u)\bigtriangleup N^+(v)|\leq \theta(|V'|)$}{
                        Include $u,v$ in the same cluster\;
                    }
          
          }
      Include all clusters formed in this step that have size at least $N/k$.\; 
      Remove all vertices in such clusters from $V'$ and any edge incident on them from $E'$.
      }
      \Phasethree{Growing the \emph{active} cluster set.\;
      \For{every unassigned vertex $v\in V\backslash V'$}{
      \For{every cluster $\mathcal{C}\in$ active}{
        Randomly pick $c\log(n)$ distinct vertices from $\mathcal{C}$ and query $v$ with them.\;
        \uIf{the majority answers are yes}{include $v$ in $\mathcal{C}$\;
        Break the loop and continue to another unassigned vertex.
        }
      }
      }
      If there are still points in $V\backslash V'$, move to Phase 1 to obtain the remaining clusters.
      }
  }
\end{algorithm2e}

==> pfthm_noisy.tex <==
Now we will prove theorem~\ref{thm:QKMwNoise}. Our proof will rely on the theoretical guarantee for the Algorithm 2 in \cite{mazumdar2017clustering}, which says the following
\begin{theorem}[Theorem 3 in \cite{mazumdar2017clustering}]\label{thm:arya1}
   Given a set of $M$ points $\mathcal{X}'$ which can be partition into $K$ clusters $\mathcal{X}' = \bigcup_{i = 1}^{K}S_i^{\dagger}$. Let $N = \frac{64K^2\log M}{(1-2p)^4}$. The Algorithm 2 in \cite{mazumdar2017clustering} will return all clusters of size at least $\frac{64K\log M}{(1-2p)^4}$ with probability at least $1-\frac{2}{M}$. The query complexity is $O(\frac{M K^2\log M}{(1-2p)^4})$ and the running time will be $O(\frac{MK\log M}{(1-2p)^2}+KN^{\omega})$ where $\omega \leq 2.373$ is the exponent of fast matrix multiplication.
\end{theorem}
Moreover, we shall modified lemma~\ref{lma:Inaba} for the without replacement case. Which means the following
\begin{lemma}[The without replacement case of Lemma 2 in \cite{inaba1994applications}]\label{lma:modified_Inaba}
Let $S$ be a set of points obtained by sampling $m$ points (without replacement) uniformly at random with replacement from a point set $A$. Then for any $\delta > 0$, with probability at least $1-\delta$
\begin{equation*}
    \phi(\mathcal{A};\mu(S)) \leq (1+\frac{1-\frac{m-1}{|A|-1}}{\delta m})\phi_1^*(\mathcal{A}) \leq (1+\frac{1}{\delta m})\phi_1^*(\mathcal{A})
\end{equation*}
Here $\mu(S)$ means the average of $S$ or says the mass center of $S$. We require $m\leq |A|$.
\end{lemma}
\begin{proof}
  Let $S = \{y_1,...,y_m\}$ be the set of $m$ points we sampled. Let $\E_{\bar{y}}$ denote the expectation with respect to $y_1,...,y_m$. Similarly by bias variance decomposition we have
  \begin{equation*}
     \sum_{x\in \mathcal{A}}||x-\mu(S)||^2 = \sum_{x\in \mathcal{A}}||x - \mu(\mathcal{A})||^2 + |\mathcal{A}|\cdot ||\mu(S)- \mu(\mathcal{A})||^2
  \end{equation*}
  Now we would like to analyze $\E_{\bar{y}}||\mu(S)- \mu(\mathcal{A})||^2$ in order to use Markov's inequality. By definition we have\
  \begin{equation*}
    \begin{split}
         & \E_{\bar{y}}||\mu(S)- \mu(\mathcal{A})||^2 = \E_{\bar{y}}||\frac{1}{m}\sum_{i=1}^{m}(y_i- \mu(\mathcal{A}))||^2 = \frac{1}{m^2}\E_{\bar{y}}||\sum_{i=1}^{m}(y_i- \mu(\mathcal{A}))||^2 \\
         & = \frac{1}{m^2}\E_{\bar{y}}(\sum_{i=1}^{m}||(y_i- \mu(\mathcal{A}))||^2+\sum_{i\neq j}\ip{y_i- \mu(\mathcal{A})}{y_j- \mu(\mathcal{A})})\\
         & = \frac{1}{m^2}(\sum_{i=1}^{m}\E_{\bar{y}}||(y_i- \mu(\mathcal{A}))||^2+\sum_{i\neq j}\E_{\bar{y}}\ip{y_i- \mu(\mathcal{A})}{y_j- \mu(\mathcal{A})})\\
         & = \frac{1}{m^2}(m\phi^*(\mathcal{A})+\sum_{i\neq j}\E_{y_i}\ip{y_i- \mu(\mathcal{A})}{\E_{y_j|y_i}(y_j- \mu(\mathcal{A}))})\\
    \end{split}
  \end{equation*}
  Note that
  \begin{equation*}
    \begin{split}
         & \E_{y_j|y_i}(y_j- \mu(\mathcal{A})) = \frac{1}{|A|-1}\sum_{y_j\in\mathcal{A}/\{y_i\}}((y_j- \mu(\mathcal{A})) \\
         & = \frac{1}{|\mathcal{A}|-1}(|\mathcal{A}|\mu(\mathcal{A})-y_i-(|\mathcal{A}|-1)\mu(\mathcal{A})) = \frac{-1}{|\mathcal{A}|-1}(y_i-\mu(\mathcal{A}))
    \end{split}
  \end{equation*}
  Hence we have
  \begin{equation*}
    \begin{split}
         & \frac{1}{m^2}(m\phi^*(\mathcal{A})+\sum_{i\neq j}\E_{y_i}\ip{y_i- \mu(\mathcal{A})}{\E_{y_j|y_i}(y_j- \mu(\mathcal{A}))})\\
         & = \frac{1}{m^2}(m\phi^*(\mathcal{A})+\sum_{i\neq j}\E_{y_i}\ip{y_i- \mu(\mathcal{A})}{\frac{-1}{|\mathcal{A}|-1}(y_i-\mu(\mathcal{A}))}) \\
         & = \frac{1}{m^2}(m\phi^*(\mathcal{A})-\frac{1}{|\mathcal{A}|-1}\sum_{i\neq j}\E_{y_i}||y_i- \mu(\mathcal{A})||^2) \\
         & = \frac{1}{m^2}(m\phi^*(\mathcal{A})-\frac{1}{|\mathcal{A}|-1}m(m-1)\phi^*(\mathcal{A})) \\
         & = \frac{\phi^*(\mathcal{A})}{m}(1-\frac{(m-1)}{|\mathcal{A}|-1}) \\
    \end{split}
  \end{equation*}
  Hence combine all the equations above and by Markov's inequality we complete the proof.
\end{proof}
Finally, we will use the following lemma
\begin{lemma}\label{lma:KLbound}
    Let's denote $D(x||y)$ be the KL divergence of Bernoulli distribution with parameter $x\leq y \in [0,1]$ respectively. We have
    \begin{equation}
       D(x||y) \leq \frac{(y-x)^2}{2y}
    \end{equation}
\end{lemma}
\begin{remark}
    Note that the bound is tighter than directly using Pinsker's inequality when $y\leq 1/4$. This bound can be found on wiki but without reference and proof. I'll give the proof for completeness.
\end{remark}
\begin{proof}
    By definition we have $D(x||y) = x\log \frac{x}{y} + (1-x)\log \frac{1-x}{1-y}$. Then note that we have the following to lower bound for log
    \begin{equation*}
       \begin{split}
            & \log(1+z) \geq z-\frac{z^2}{2} \;\forall |z|<1 \\
            & \log(z) \geq 1-\frac{1}{z}\;\forall z>0
       \end{split}
    \end{equation*}
    We can see them directly by Taylor expansion. Hence applying the first inequality to $\log(\frac{x}{y})$ and the second to $\log\frac{1-x}{1-y}$ we have
    \begin{equation*}
      \begin{split}
           & D(x||y) \geq x(\frac{x-y}{y}-\frac{(x-y)^2}{2y^2}) + (1-x)(1-\frac{1-y}{1-x}) \\
           & = -\frac{x}{2}\frac{(y-x)^2}{y^2}+(y-x)(1-\frac{x}{y}) \\
           & = \frac{(y-x)^2}{y}(1-\frac{x}{2y}) \\
           & \geq \frac{(y-x)^2}{y}(1-\frac{1}{2})\;\text{Since }x\leq y\in[0,1] \\
           & = \frac{(y-x)^2}{2y}
      \end{split}
    \end{equation*}
\end{proof}
Now we're ready to proof theorem~\ref{thm:QKMwNoise}.
\begin{proof}
  For the correctness, we first see that if we uniformly at random sample $M$ points from $\mathcal{X}$, we will get a new set $\mathcal{X}'$. Note that $\mathcal{X}'$ can still be partition into $K$ clusters $\forall i\in[K], S_i^\dagger = \mathcal{X}'\bigcap \mathcal{C}_i^*$. Since we uniformly at random sample points, hence the vector $(S_1^\dagger,...,S_K^\dagger)$ is multivariate hypergeometric random vector with parameters$(n,np_1,...,np_K,M)$ where $p_i=\frac{|S_i^*|}{n}\forall i\in[K]$. Moreover, we denote $p^* = \min_{i}p_i = \frac{1}{\alpha K}$ by the $\alpha$-balance property. Now we focus for $S_i^\dagger$, which is a hypergeometric random variable with parameter $(n,np_i,M)$. It's well known (\cite{hoeffding1963probability}, \cite{skala2013hypergeometric}) that the tail bound of it is (Denote $D(p||q)$ be the KL divergence of Bernoulli distribution with parameter $p,q$ respectively)
  \begin{equation}\label{pfthm:hypergeotailbound}
     \begin{split}
          & P(S_i^\dagger < M(p_i-\frac{p_i}{2})) \leq \exp(-MD(\frac{p_i}{2}||p_i)) \leq \exp(-\frac{Mp_i}{8}) \\
          & \Rightarrow P(S_i^\dagger  < \frac{Mp_i}{2}) \leq \exp(-\frac{Mp_i}{8}) \\
          & \Rightarrow P(S_i^\dagger  < \frac{Mp^*}{2}) \leq \exp(-\frac{Mp^*}{8}) \\
     \end{split}
  \end{equation}
  Where we use the fact $D((1-x)p||p)\geq \frac{1}{2}x^2p,\;x\in[0,\frac{1}{2}]$, which is the direct result of lemma~\ref{lma:KLbound}. Hence by union bound over $K$ we have
  \begin{equation}\label{pfthm:QKMwNoise_Chernoff2}
     P(\min S_i^\dagger \geq \frac{Mp^*}{2}) \geq 1 - K\exp(-\frac{Mp^*}{8})
  \end{equation}
  Now we require $\min S_i^\dagger$ to be at least $\max\{\frac{64K\log M}{(2p-1)^4},\frac{3K}{\delta \epsilon}\}$, this correspond to \eqref{Mcondi} and the first term in \eqref{M1condi}. The first term in max is because we want to satisfy the requirement in theorem~\ref{thm:arya1}. The second term in max is because we want to apply lemma~\ref{lma:Inaba}. By the choice of our $M$ we can make sure this two requirements holds. Also, we want the statement hold with probability at least $1-\frac{\delta}{3}$, which will need $M\geq 8\alpha K\log \frac{3K}{\delta}$. This correspond the second term in \eqref{M1condi}. By our choice of $M$ this will also holds. Then by theorem~\ref{thm:arya1}, we know that after phase 1, we will get the underlying optimal partition $S_1^\dagger,...,S_K^\dagger$ with probability at least $1-\frac{2}{M}$. By our choice of $M$ we can make sure this probability is at least $1-\frac{\delta}{3}$. Finally, since every points in $S_1^\dagger,...,S_K^\dagger$ is uniformly at random sampled from $\mathcal{X}$, thus by applying lemma~\ref{lma:modified_Inaba}, union bound and by our choice of $M$ we know that with probability at least $1-\frac{\delta}{3}$, the resulting set of centers $\mathcal{C}$ will achieve the $(1+\epsilon)$-approximation. Finally by union bound over all error events, we know that with probability at least $1-\delta$, $\mathcal{C}$ will achieve the $(1+\epsilon)$-approximation. For the query complexity and the time complexity, it directly follows the result of theorem~\ref{thm:arya1}. Hence we complete the proof.
\end{proof} 

==> pfthm_outliers.tex <==
We first argue that theorem~\ref{thm:QKMwOL} is a $(1+\epsilon)$ approximation algorithm with probability at least $(1-\delta)$. Note that by the construction of Phase 1 in algorithm~\ref{alg:QKMwOL}, we can ensure that the clusters $\mathcal{S}$ containing $K$ pairs points are all non-outliers and each pairs are from different optimal cluster. Hence after Phase 2, by theorem~\ref{thm:ourmain}, we know that theorem~\ref{thm:QKMwOL} indeed is a $(1+\epsilon)$ approximation algorithm with probability at least $(1-\delta)$.\\
Next we're going to prove the bound of expected query complexity $\E Q$. We first decompose $Q$ into $Q_1$, the query complexity of Phase 1 and $Q_2$, the query complexity of Phase 2. Let's first dealing with $Q_1$. Again by poissonization argument, we can denote the number of points we sample in Phase 1 at time $t$ as $Z(t)\sim Poisson(t)$ and $Z_j(t)\sim Poisson(p_j t),j\in\{0,...,K\} $ and $Z_j(t)$ are independent poisson process. Moreover, let $X_j$ be the time that we sample $2$ point from optimal cluster $\mathcal{C}_j^*$ and $X = \max_{i\in[K]}X_i$. So we have
\begin{equation}\label{pfthm10eq1}
    \begin{split}
         & \E (Q_1) \leq \E \E (K\sum_{i=1}^{K}Z_i(X) + \sum_{j=1}^{Z_0(X)}(K+j-1)|X) \\
         &  = K\E X + \E(\frac{Z_0(X)(Z_0(X)-1)}{2}|X) = K\E X + \frac{p_0^2}{2}\E X^2
    \end{split}
\end{equation}
The inequality is true since when we sample a point from $\mathcal{X}_t$, then we will at most use $K$ queries in that round. This will result the first term $K\sum_{i=1}^{K}Z_i(X)$. When we sample a point from $\mathcal{X}_o$, assuming we have already sample $a$ outliers, then for this point we will at most use $K+a$ queries. Hence this will result the second term $\sum_{j=1}^{Z_0(X)}(K+j-1)$. Now we check the bound for $\E X$ and $\E X^2$. For $\E X$, by the same trick used in the proof of theorem~\ref{thm:ourmain}, we have (note that we have $m=2$ here)
By the same trick in the proof of theorem~\ref{thm:ourmain} we have ($\lambda = \frac{p^*}{2}\in (0,p^* = \min p_i)$)
\begin{equation}\label{pfthm10eq3.1}
    \begin{split}
         & \E X = \E \max_{i\in[K]}X_i \\
         & \leq \frac{1}{\lambda}\log\sum_{i=1}^{K} \E \exp(\lambda X_i)\\
         & = \frac{1}{\lambda}\log\sum_{i=1}^{K} (\frac{p_i}{p_i-\lambda})^m \leq \frac{2}{p^*}\log (K2^m)\\
         & \leq \frac{2\alpha K}{1-p_0}(\log K + 2\log2)
    \end{split}
\end{equation}
Where the last equality is from the $\alpha$-balance property and $m = 2$ by the construction of algorithm.
For the second moment, however we're not able to apply the same trick since $\E exp(X_j^2)$ doesn't exist (It's infinite since $X_j$ is not subgaussian, it's sub-exponential instead). Hence we have to deal with it in a more careful way. $\forall t\in(0,p^*)$, we have
\begin{equation*}
    \begin{split}
         & \E X^2 = \E (\max_{i\in[K]}X_i)^2 \\
         & = \E\frac{1}{t^2}(\log(\exp(t\max X_i^2)))^2 \\
         & = \E\frac{1}{t^2}(\log(\max \exp(t X_i^2)))^2
    \end{split}
\end{equation*}
Now, we note that $(\log x)^2$ is concave over $x\in[e,\infty)$ and it's monototic non-decreasing, hence
\begin{equation}\label{pfthm10eq3.2}
   \begin{split}
         & = \E\frac{1}{t^2}(\log(\max \exp(t X_i)))^2\\
         & \leq \E\frac{1}{t^2}(\log((\max \exp(t X_i))\mathbf{1}(\max tX_i \geq 1)+e\mathbf{1}(\max tX_i < 1)))^2\\
         & \leq \E\frac{1}{t^2}(\log((\max \exp(t X_i))+e))^2\\
         & \leq \frac{1}{t^2}(\log(\E(\max \exp(t X_i))+e))^2 \;\text{By Jensen's inequality}\\
         & \leq \frac{1}{t^2}(\log(\sum_{i=1}^{K}\E(\exp(t X_i))+e))^2\\
         & = \frac{1}{t^2}(\log(\sum_{i=1}^{K}(\frac{p_i}{p_i-t})^m+e))^2\\
         & \leq \frac{4}{(p^*)^2}(\log(K2^m+e))^2 \; \text{Take }t=\frac{p^*}{2}\\
         & \leq (\frac{2\alpha K}{1-p_0}\log(K2^m+e))^2\\
         & \leq (\frac{2\alpha K}{1-p_0}\log(2K2^m))^2 \;\text{Assume }K2^m\geq e\\
         & = (\frac{2\alpha K}{1-p_0}(\log(2K)+m\log2))^2
    \end{split}
\end{equation}
Note that now $m=2$ hence obviously we have $K2^m= 4K \geq 4 \geq e$. Now we can plug in $m=2$ into \eqref{pfthm10eq3.2} and plug \eqref{pfthm10eq3.2} ,\eqref{pfthm10eq3.1} into \eqref{pfthm10eq1}, we have
\begin{equation}\label{pfthm10eq4}
   \E (Q_1) \leq  K\E X + \frac{p_0^2}{2}\E X^2 \leq \frac{2\alpha K^2}{1-p_0}(\log K + 2\log 2)+2(\frac{\alpha K p_0}{1-p_0}(\log(2K)+2\log2))^2
\end{equation}
For $Q_2$, we can still follow the similar analysis as the proof in theorem~\ref{thm:ourmain} and above. By the same poissonization argument in the proof of theorem~\ref{thm:ourmain}, we can denote the number of points we sample in Phase 2 at time $t$ as $Z(t)\sim Poisson(t)$ and $Z_j(t)\sim Poisson(p_j t),j\in\{0,...,K\} $ and $Z_j(t)$ are independent poisson process. Let $X_j$ be the time that we sample $m$ points from $\mathcal{C}_j^*$ for $j\in\{1,...,K\}$ and $X=\max_{i\in[K]}X_i$. Note that $X_j\sim Erlang(m,p_j)$ independently. Then we have
\begin{equation}\label{pfthm9eq4}
   \E (Q_2) \leq \E\E (Z_0(X) + K\sum_{i=1}^{K}Z_i(X)|X) = (p_0+K(1-p_0))\E X
\end{equation}
Since $X = \max_{i\in[K]}X_i$ is independent of $Z_0$ and $Z_0$ is Poisson, hence the first term is $\E p_0 X$. The second term is by the fact that
\begin{equation*}
  \text{Let } Y=\sum_{i=1}^{K}Z_i(X), \E X = \E \sum_{i=1}^{Y} U_i = \frac{1}{1-p_0}\E Y,\text{ where }U_i\text{ are iid exponential with rate } 1-p_0
\end{equation*}
Then plug in \eqref{thm5eq1.1} with $m = \frac{K}{\delta \epsilon}$, we have
\begin{equation}\label{pfthm10eq5}
   \E Q_2 \leq \frac{2\alpha K}{1-p_0}(p_0+K(1-p_0))(\log K + (\frac{K}{\delta \epsilon}-2)\log2)
\end{equation}
Hence together we have
\begin{equation}\label{pfthm10eq6}
    \begin{split}
         & \E Q \leq \frac{2\alpha K^2}{1-p_0}(\log K + 2\log 2)+2(\frac{\alpha K p_0}{1-p_0}(\log(2K)+2\log2))^2 \\
         & + \frac{2\alpha K}{1-p_0}(p_0+K(1-p_0))(\log K + (\frac{K}{\delta \epsilon}-2)\log2)
    \end{split}
\end{equation}
Hence we complete the proof.

==> sec_comp.tex <==
The work \cite{gamlath2018semi} focus on an extension where they can also guarantee that the resulting clustering for their algorithm can not only achieve $(1+\epsilon)$ approximation with high probability but also ensure that the misclassification ratio is less than $\epsilon$. As a result, their method will require more query complexity to achieve this harder requirement compare to \cite{ailon2017approximate}. Moreover, they extend the problem setting to finite metric space. However, they only consider the case with noiseless oracle. In contrast we consider not only the noisy oracle case, but also the case with outliers. At last, since our method need less queries under a mild assumption of the smallest cluster size compare to \cite{ailon2017approximate}, the query complexity of our method is also superior to theirs.\\
The work \cite{kim2017semi} is more closely related to the work of \cite{ashtiani2016clustering}. They focus on exact recovery with a weak oracle which is different from \cite{ashtiani2016clustering}. Basically they says the weak oracle will randomly abstain from giving an answer to queries (i.e. reply "I don't know"). They show that under the same $\gamma$-margin assumption their method can superior to the result of \cite{ashtiani2016clustering} when the oracle is not weak. They also show the results for the several types of weak oracle with some additional assumptions. In contrast, our work focus on finding an $(1+\epsilon)$ approximation. Moreover, we consider both the cases of noisy oracle and outliers which is different from theirs.\\
The rest two papers \cite{kane2017active}, \cite{tosh2018structural} seems to be more irrelevant to ours... 

==> sec_probform.tex <==
%\subsection{Background}
We start with a formal definition of the K-means problem.

    Given a set of $n$ points $\mathcal{X} \subset \mathbb{R}^d,$ and a number of clusters K, the K-means problem asks for finding a set of points $\mathcal{C}=\{c_1,...,c_K\}\subset \mathbb{R}^d$ that minimizes the following objective function
    \begin{equation*}
       \phi(\mathcal{X};\mathcal{C}) = \sum_{x\in \mathcal{X}}\min_{c\in\mathcal{C}}||x-c||^2,
    \end{equation*}
    where $||\cdot||$ denotes the $L_2$ norm. Throughout the paper, we assume that the optimal solution is unique, and denote it by $\mathcal{C}^* = \{c_1^*,...,c_K^*\}$. The set of centroids $\mathcal{C}^*$ induces an optimal partition $\mathcal{X} = \bigcup_{i=1}^{K}\mathcal{C}_i^*$, where $\forall i\in[K], \mathcal{C}_i^* = \{x\in\mathcal{X}: ||x-c_i^*||\leq ||x-c_j^*||\;\forall j\neq i\}$. We also use $\phi_K^*(\mathcal{X})$ to denote the optimal value of the objective function.
    %value for point set $\mathcal{X}$ with $K$ centers. Also we will use $[K]$ to denote the set $\{1,...,K\}$.

As already stated, the K-means clustering problem is NP-hard, and hard to approximate within a $(1+\epsilon)$ factor, for $0<\epsilon<1$. An important question in the approximate clustering setting was addressed by Inaba et al.~\cite{inaba1994applications}, who showed how many points from a set have to be sampled uniformly at random to guarantee, that for any $\epsilon>0$ and with high probability, the centroid of the set can be estimated within a multiplicative $(1+\epsilon)$-term. This results was used by Ailon et.al~\cite{} in the second (sub)sampling procedure. In our work, we make use of the same result in order to determine the smallest number of points (coupons) one needs to collect for each cluster (coupon type).
\begin{lemma}[Centroid lemma, Lemma 2 of~\cite{inaba1994applications}]\label{lma:Inaba}
Let $A$ be a set of points obtained by sampling with replacement $m$ points independently from each other, uniformly at random, from a point set $S$. 
Then, for any $\delta > 0$, one has
\begin{equation*}
   P(\phi(\mathcal{S};c(A)) \leq (1+\frac{1}{\delta m})\phi^*(\mathcal{S})) \geq 1-\delta,
\end{equation*}
where $c(A)$ stands for the centroid of $A$.
\end{lemma}
The Centroid lemma is used in conjunction with a generalization of the double Dixie cup problem to establish the described query complexity results in the noiseless setting. The double Dixie cup problem is an extension of the classical coupon collector problem in which the collector is required to collect $m \geq 2$ sets of coupons. While the classical coupon collector problem may be analyzed using elementary probabilistic tools, the double Dixie cup problem solution requires using generating functions and complex analysis techniques. For the most basic incarnation of the problem where each coupon type is equally likely and each coupon needs to be collected at least $m$ times, where $m$ is a constant, Newman and Shepp~\cite{newman1960double} showed that one needs to purchase $O(K(\log K + (m-1)\log\log K))$ coupons. This setting is inadequate for our analysis, as our coupons represent points from different clusters that have different sizes, and hence give rise to different coupon (cluster point) probabilities. Furthermore, in our analysis we require $m = \frac{K}{\delta \epsilon}$, which scales with $K$ and is significantly harder to analyze. The starting point of our generalizations of nonuniform probability double Dixie cup problem is the work of Doumas~\cite{doumas2016coupon}. We extend the Poissonization argument and perform a careful analysis of the expectation of the maximum order statistics of  of independent random variables distributed according to the Erlang distribution. All technical details are delegated to the Supplement. 

Often, one seeks the K-means solutions in a setting where the cluster points $\mathcal{X}$ satisfy certain separability and cluster size constraints, such as the $\gamma$-margin and the bounded minimum cluster size constraint, respectively. Both are formally defined below. 
\begin{definition}[The $\gamma$-margin property~\cite{ashtiani2016clustering}]
   Let $\gamma>1$ be a real number. We say that $\mathcal{X}$ satisfies the $\gamma$-margin property if $\forall \, i\neq j \in [K], \, x\in \mathcal{C}_i^*,\, y\in \mathcal{C}_j^*,$ one has
   \begin{equation*}
      \gamma ||x-c_i^*|| < ||y-c_i^*||.
   \end{equation*}
\end{definition} 
To describe the cluster size constraint, we introduce the notion of $\alpha$-balance.
\begin{definition}[The $\alpha$-balance property]
Let $\alpha \in [1,n/K]$ be a real number. We say that the point set $\mathcal{X}$ satisfies the $\alpha$-balance property if $\alpha=\frac{n}{K\, s_{\text{min}}}$.
\end{definition}
To avoid complicated and costly two-level queries, we impose an $\alpha$-balance constraint on the optimal clustering excluding outliers.

For the outliers, we use a milder version of the $\gamma$-margin constraint, described as follows. Assume that $\mathcal{X}=\mathcal{X}_t \cup \mathcal{X}_o$, where $\mathcal{X}_t$ and $\mathcal{X}_o$ are the nonintersecting sets of true cluster points and outliers, respectively. Outliers are formally defined as follows.
\begin{definition}
   The set $\mathcal{X}_o$ consists of points that satisfy the $\Gamma(\epsilon)$-separation property, defined as
    \begin{equation*}
        \forall x\in \mathcal{X}_o, \, \forall \; i\in[K],\; ||x-c_i^*|| > \max_{y\in C_i^*}||y-c_i^*||+\sqrt{\frac{\epsilon \, \phi^*(C_i^*)}{|C_i^*|}} \geq \Gamma(\epsilon).
    \end{equation*}
Here, $\Gamma(\epsilon)$ is the smallest positive value that satisfies the lower bound for all values of $i\in[K]$.
\end{definition}
This is a reasonable modeling assumption, as outliers by definition lie in ``clusters'' that are well-separated from all ``regular'' clusters. In this extended setting, the  objective is to minimize the function $\phi(\mathcal{X}_t,\mathcal{C})$. Furthermore, with a slight abuse of notation, we use $C_1^*,...,C_K^*$ to denote 
both the optimal partition for $\mathcal{X}_t$ and $\mathcal{X}$. It should be clear from the context which clusters are referred to.

Side information for the K-means problem is provided by a query oracle $\mathcal{O}$ such that  
\begin{equation}\label{oracle1}
   \forall x_1,x_2\in\mathcal{X}, \;\mathcal{O}(x_1,x_2) =
   \begin{cases}
     0, & \mbox{if } \, \exists i \, \in[K]\; \text{s.t. } x_1\in C_i^*, x_2\in C_i^*; \\
     1, & \mbox{otherwise}.
   \end{cases}
\end{equation}
Query complexity is measured in terms of the number of time that an algorithm is given access to the oracle. 
The goal is to devise query algorithms with query complexity as small as possible. 
%Our goal is to design an algorithm that can interact with the oracle $\mathcal{O}$. 
%We hope to output a set of centers with objective function value ($\phi(\mathcal{X},\mathcal{C})$) as low as possible and with query complexity as low as possible. 
The noisy oracle $\mathcal{O}_n$ may be viewed as the response of a binary symmetry channel with parameter $p$ to an input produced 
by the perfect oracle $\mathcal{O}$. Equivalently, $\forall x_1,x_2\in\mathcal{X}$, $P(\mathcal{O}_n(x_1,x_2)= \mathcal{O}(x_1,x_2)) = 1-p$, and $P(\mathcal{O}_n(x_1,x_2) \neq \mathcal{O}(x_1,x_2)) = p$, independently from other queries. Each pair $(x_1,x_2)$ is queried only once, and the noisy oracle 
$\mathcal{O}_n$ always produces the same answer for the same query. When presented with at least one outlier point in the pair $(x_1,x_2)$, 
the perfect oracle always returns $\mathcal{O}(x_1,x_2)=1$, while the noisy oracle $\mathcal{O}_n$ may flip the answer with probability $p$. The problem of identifying outliers placed in regular clusters is resolved by invoking the algorithm of~\cite{mazumdar2017clustering}, which places outliers into small clusters 
that are expurgated from the list of valid clusters. 

%For our analysis, instead of requiring the $\gamma$-margin property as \cite{ashtiani2016clustering}, we introduce the $\alpha$-balance property to characterize the balance among the size of optimal clusters $\mathcal{S}_1^*,...,\mathcal{S}_K^*$.
%\begin{definition}[$\alpha$-balance property]
%   Let $\alpha \in [1,\frac{n}{K}]$ be a real number. We say the $n$ point set $\mathcal{X}$ satisfies $\alpha$-balance property iff $\min_{i\in[K]}\frac{|\mathcal{S}_i^*|}{n} = \frac{1}{\alpha K}$
%\end{definition}
%In \cite{ashtiani2016clustering}, they define a way to characterize the separation of $\mathcal{X}$, which they call the $\gamma$-margin property.
%They first show that for $\gamma \in(1,\sqrt{3.4}]$ and $K = \Theta(n^{\eta})$ for any $\eta\in(0,1)$, solving Kmeans exactly is still NP-hard. Then they show that under the SSCA setting, they provide an algorithm which can solve the Kmeans problem with high probability. The formal statement is as following
%\begin{theorem}[Theorems 7 and 8 in \cite{ashtiani2016clustering}]\label{thm:2016nips}
%Let $\delta\in(0,1)$ and $\gamma > 1$. Given a set of $n$ points $\mathcal{X}$, an integer $K$ and assuming $\mathcal{X}$ satisfying $\gamma$-margin property. Then there is an query algorithm $A$ that makes $O(K\log n + K^2\frac{\log K + \log(1/\delta)}{(\gamma-1)^4})$ same-cluster queries and with probability at least $1-\delta$ output the optimal partition $\mathcal{S}_1^*,...,\mathcal{S}_K^*$. The time complexity of algorithm $A$ is $O(Kdn\log n+K^2\frac{\log K + \log(1/\delta)}{(\gamma-1)^4})$.
%\end{theorem}
%From the above theorem, we could see that using only $O(K\log n + K^2\frac{\log K + \log(1/\delta)}{(\gamma-1)^4})$ same-cluster queries, we can solve the Kmeans problem exactly with high probability even in the regime that it's NP-hard. This shows that the using same-cluster queries as the side information is indeed powerful.\\
%On the other hand, \cite{ailon2017approximate} provides a sophisticate algorithm to solve the Kmeans problem approximately with high probability. Note that they do not make the $\gamma$-margin property assumption. The formal statement of their result is as following
%\begin{theorem}[Theorem 3 in \cite{ailon2017approximate}]\label{thm:ailon}
%  Let $\epsilon\in(0,0.5)$, $K$ be any natural and a set of $n$ points $\mathcal{X}\subset \mathbb{R}^d$. Then there is a query algorithm $A$ that runs in time $O(\frac{ndK^9}{\epsilon^4})$ and with probability at least $0.99$ outputs a center set $\mathcal{C}$ such that $\phi(\mathcal{X};\mathcal{C})\leq (1+\epsilon)\phi_K^*(\mathcal{X})$.  Moreover, the query complexity of algorithm $A$ is $O(\frac{K^9}{\epsilon^4})$.
%\end{theorem}

==> subsec_toprcluster.tex <==
Due to the space limitation, we will put the algorithm in the appendix and only state the theorem. We denote the ratio of the size of cluster $|S_i^*|$ to $n$ as $p_i = \frac{|S_i^*|}{n}$. Without loss of generality we assume $p_i$ are also sorted. Then we define $\bar{p} = \frac{p_r+p_{r+1}}{2}$ and $\Delta = p_r -\bar{p}$. Moreover, let $KL(a||b)$ be the KL-divergence for Bernoulli($a$) and Bernoulli($b$). We denote $D = \min\{KL(\bar{p}||\bar{p}+\Delta),KL(\bar{p}||\bar{p}-\Delta)\}$
\begin{theorem}\label{thm:toprclusters}
    Assume that $\bar{p}\in(0,1)$ and $\Delta > 0$. Let us denote $\tilde{p} = \sum_{i=1}^{r}p_i$.
    Then exist an algorithm which will output a set of centers $\mathcal{C}$ such that with probability at least $1-\delta$, $\phi(\mathcal{X}^{(r)};\mathcal{C})\leq (1+\epsilon)\phi^*(\mathcal{X}^{(r)})$. The expected query complexity $\E Q$ can be bounded as
    \begin{equation*}
       \E Q \leq \frac{K}{D}\log\frac{2K}{\delta} + \frac{2}{p_r}(1-\tilde{p}+K\tilde{p})(\log K +\frac{2K}{\delta \epsilon}\log 2)
    \end{equation*}
    Moreover, the expected time complexity for outputting $\mathcal{C}$ is $O(\E Q)$.
\end{theorem}
\begin{remark}
    The first term in the query complexity upper bound is the query complexity for Phase 1, which is clearly $KM = \frac{K}{D}\log\frac{2K}{\delta}$ by our choice of $M$. The second term will be similar to the case as theorem~\ref{thm:QKMwOL}. Note that our bound here should be able to further be refined since the bound we use for phase 2 here is to collecting $\frac{2K}{\delta \epsilon}$ for all top $r$ largest clusters starting with 1 points for each clusters. However for simplicity we present the looser bound here.
\end{remark}
The proof can be found in the appendix.
